Spectrum Sharing For Information Freshness: A Repeated Games Perspective

We consider selfish sources that send updates to a monitor over a shared wireless access. The sources would like to minimize the age of their information at the monitor. Our goal is to devise strategies that incentivize such sources to use the shared spectrum cooperatively. Earlier work has modeled such a setting using a non-cooperative one-shot game, played over a single access slot, and has shown that under certain access settings the dominant strategy of each source is to transmit in any slot, resulting in packet collisions between the sources' transmissions and causing all of them to be decoded in error at the monitor. We capture the interaction of the sources over an infinitely many medium access slots using infinitely repeated games. We investigate strategies that enable cooperation resulting in an efficient use of the wireless access, while disincentivizing any source from unilaterally deviating from the strategy. Formally, we are interested in strategies that are a subgame perfect Nash equilibrium (SPNE). We begin by investigating the properties of the one-stage (slot) optimal and access-fair correlated strategies. We then consider their many-slot variants, the age-fair and access-fair strategies, in the infinitely repeated game model. We prove that the access-fair and age-fair strategies are SPNEs for when collision slots are longer than successful transmission slots. Otherwise, neither is a SPNE. We end with simulations that shed light on a possible SPNE for the latter case.

==> stage_game.tex <==
\section{Single stage game}
We propose a cooperation strategy for the selfish nodes (that care to minimize their age of the information), where a centralized mechanism dictates the node's actions. For example, it would select the node that would transmit in a given slot, and others would sit idle, or it might not select any node resulting in an idle slot. If any node/nodes deviate from this plan, a grim trigger punishment would be activated, where all nodes would play the minmax strategy for the rest of the slots. We also found the minmax payoff for node k corresponding to the strategy where at least two nodes transmit is $-(\Delta_ + \sigma_C)$. According to Folk's theorem, A strategy with payoffs greater than or equal to minmax payoffs can be played as cooperation over repeated games. We want to find an optimal strategy with payoffs greater than the minmax payoff while minimizing the network's cumulative expected ages.

We next look at how the centralized unit would choose an action plan for all the nodes keeping in mind that the strategy should result in a payoff from the feasible payoff set and should minimize the network's cumulative age as given in the optimization formulation below.
 Let $P_k$ denote the probability of selecting a strategy where node k transmits successfully, i.e., only node k transmits while the remaining nodes stay idle. When such an event occurs, the age of the node k resets to $\sigma_S$, while the age of the remaining nodes increases by $\sigma_S$. Let $P_I$ be the probability of an idle slot, i.e., no node transmits, and the age of each node increase by $\sigma_I$. Lastly, let $P_C$ be the probability of a collision, i.e., two or more nodes transmit, and the age of each node increases by $\sigma_C$. The optimization problem is formulated as an objective function (sum of expected age of all the nodes in the network), Constraint 1(Expected payoff for each node is greater than or equal to the minmax payoffs), and Constraint 2(Probabilities of picking up one of the strategies is non-negative and sums up to 1).
\\
$\textbf{Minimize}_{P_k,P_I,P_C} \sum_{k=1}^{N} E[U_k(P_k,P_I,P_C)]$\\
such that: $E[U_k((P_k,P_I,P_C)] \geq U_{k,Minmax}$, and $P_k,P_I,P_C \geq 0; \sum_{k=1}^{N} P_k + P_I + P_C = 1$\\

$\sum_{k=1}^{N} E[U_k(P_k,P_I,P_C)] =  \sum_{k=1}^{N} [P_k\sigma_{S} + P_I(\Delta_{k}+\sigma_{I}) +  P_C (\Delta_{k}+\sigma_{C}) + \sum_{j=1, j\ne k}^{N} p_{t_{j}}(\Delta_{k} + \sigma_{S})]$\\
\\
We minimize the variable corresponding to the maximum coefficient to minimize the linear objective function. By this logic, we can say that $P_C = 0$. 
Proof: Suppose some probability vector $(P_1,P_2,..,P_N,P_C,P_I)$ that satisfies the constraints was optimal with $P_C > 0 $, then shifting weight from $P_C = 0$ to $P_I = P_C + P_I$, i.e., another vector $(P_1,P_2,..,P_K,0, P_C + P_I)$ is in the feasible set and contradicts by achieving lower objective function value than the optimal vector $(P_1,P_2,..,P_K,P_C,P_I)$ because $\sum_{k=1}^{N}\Delta_k + N\sigma_C > \sum_{k=1}^{N}\Delta_k + N\sigma_I$. Therefore $P_C$ will always be 0. Further, We look at the coefficient corresponding to $P_I$. It is minimum if and only if $\Delta_k < N(\sigma_S - \sigma_I)$ $\forall k \in [1,N]$. If this were true, the optimal strategy would be to maximize the probability of choosing the strategy where no node transmits. Note this condition can only be true if a new node is introduced in the network and its initial age satisfies the above condition. this can be explained as no two nodes could successfully transmit in the same slot. We analyze the optimal strategy for two different MAC settings. 1) Basic access where $\sigma_S > \sigma_C$, and 2) RTS/CTS based where $\sigma_S \leq \sigma_C$\\
\\
\\

\textbf{1) Basic Access Mechanism $\sigma_S < \sigma_C$:} \\
2-player game: The minmax payoff for node k is $\Delta_k + \sigma_S$, thus any probability vector that satisfies $P_1\sigma_S + P_2(\Delta_1 + \sigma_S) + P_I(\Delta_1 + \sigma_I) \leq (\Delta_1 + \sigma_S)$ and $P_1(\Delta_2 + \sigma_S) + P_2 \sigma_S + P_I(\Delta_2 + \sigma_I) \leq (\Delta_2 + \sigma_S)$ lies in the feasible set region. It is clear as $\Delta_k +\sigma_S \geq \Delta_k +\sigma_I \geq \sigma_S $, any probability vector ($P_1,P_2,P_C = 0,P_I)$ satisfies the constraints. Now the one with maximum age gets a chance to transmit with probability 1 as the coefficient corresponding to it is the least given that $\Delta_K > N(\sigma_S - \sigma_I)$, for at-least one node.\\

N-player game: For such a setting,  $\Delta_k + \sigma_C > \Delta_k + \sigma_S > \Delta_k + \sigma_I > \sigma_S$. Thus for every possible probability vector $(P_1, P_2, ..., P_N, P_C, P_I)$, (i.e., $ P_k \geq 0 $ $\forall k \in N$; $P_C, P_I \geq 0$; and $\sum_{k=1}^{N}P_k + P_C + P_I = 1$), constraint 1 of our optimization problem always satisfy. Since our optimization problem is minimizing over linear objective function and the constraints are bounds on probabilities, the term with minimum coefficient will be given maximum weight. By this logic, we can say that  the node with the highest age gets a chance to transmit with probability 1. If $\Delta_k < N(\sigma_S - \sigma_I)$ $\forall k \in [1,N]$, then $P_I = 1$. Thus in this scenario, a node with the highest age gets to reset its age to $\sigma_S$, thereby minimizing the cumulative network age. Another scheme of policy could be where a node is randomly picked with probability $\frac{1}{N}$, that transmits in the next slot while others sit idle. The advantage of this policy over the previous is that the centralized unit doesn't need to keep track of the ages of all the nodes in the network. This policy too, follows the constraint conditions and can also be easily implemented in practical scenarios.\\
\\

\textbf{2) RTS/CTS access $\sigma_S \geq \sigma_C$ }
\\
\\
\textbf{2 Player Game}:
We now look at the feasible set region, i.e., the region where all the constraints are satisfied. Fig. 1 shows payoffs for nodes 1 and 2 for a two-player game. The pure actions for the two-player game are (T,T), (I,T), (T,I), (I,I) corresponding to payoffs $(-\Delta_1 - \sigma_C,-\Delta_2 - \sigma_C),(-\Delta_1 - \sigma_S, -\sigma_S),(-\sigma_S,-\Delta_2 - \sigma_S),(-\Delta_1 - \sigma_I,-\Delta_2 - \sigma_I)$ respectively. We can achieve any payoff from the convex hull containing these pure strategies by playing these strategies with some probability. What I mean is any payoff set inside this convex hull is some combination of these pure strategies. Depending upon the initial ages of nodes and successful/ idle/ collision slot lengths, there can be two cases. One where the payoff corresponding to (I,I) lies below the line joining (T,I) and (I,T) as in case 1, the convex hull is triangular or where (I,I) lies above the line joining (T,I) and (I,T) as in case 2, the convex hull is quadrilateral. The feasible set constraint 1 (expected utility for each node should be greater than or equal to minmax payoff where point corresponding (T,T) represents the minmax payoff) is represented by the shaded region in fig.1. To find the optimal; we use the property of convex sets that the optimal always lies on its boundary. This helps to reduce the set we are looking at to the set of payoffs corresponding to the bold boundary lines. 
\\
\\

\begin{wrapfigure}{l}{0.25\textwidth}
\includegraphics[scale = 0.25]{figure/RTSCTS 2 player payoff regionpng.png}
\caption{2-player feasible Payoff Region for RTS/CTS access}
\end{wrapfigure}
\\

CASE 1: The payoff set corresponding to the strategy (I,I) is below the line joining payoffs for (T,I) and (I,T) as shown in Fig 1. 
\\
Equation of line: joining $(-\sigma_S, -\Delta_2 - \sigma_S$) and ($-\Delta_1 - \sigma_S, -\sigma_S$) is given by:
$y - y_1 = \frac{y_1 - y_2}{x_1 - x_2} (x - x_1)$
\\
$\Delta_2*x + \Delta_1*y = -\Delta_1 \Delta_2 - (\Delta_1 + \Delta_2)\sigma_s$
\\
payoff for I,I strategy i.e. $(-\Delta_1 -\sigma_I, -\Delta_2 -\sigma_I)$ lies below the given line if and only if 
\\
$\Delta_2*(-\Delta_1 -\sigma_I) + \Delta_1*(-\Delta_2 -\sigma_I) < -\Delta_1 \Delta_2 - (\Delta_1 + \Delta_2)\sigma_s$
\\
Hence we get the following equation
\begin{equation} \label{equation_1}
    
    
   When $\frac{\Delta_1 \Delta2}{\Delta_1 + \Delta2} \geq \sigma_s - \sigma_I$ then $P_I = 0$
    
    
\end{equation}

When this equation holds, The optimal lies on the line joining (T,I), (I,T); thus $P_I = 0$; next, we try to figure out the probabilities with which (T,I) and (I,T) are played that the expected utilities for node 1 and 2 lies in the constraint region while optimizing the objective function. With $P_C = 0, P_I = 0, P_1 + P_2 = 1$, the constraints simplify as follows:
\\
Constraint 1a: $-\sigma_S p_1 - (\Delta_1 + \sigma_S) p_2 \geq - (\Delta_1 + \sigma_C)$
\\
\implies $-\sigma_S p_1 - (\Delta_1 + \sigma_S) (1 - p_1) \geq - (\Delta_1 + \sigma_C)$
\implies $p_1\geq \frac{\sigma_S - \sigma_C}{\Delta_1}$
\\
\\
Constraint 1b: $-(\Delta_2 + \sigma_S)p_1 - \sigma_Sp_2  \geq -(\Delta_2 + \sigma_C)$\\
\implies $-(\Delta_2 + \sigma_S)p_1 - \sigma_S(1 - p_1) \geq -(\Delta_2 + \sigma_C)$ \implies $P_1 \leq \frac{\Delta_2 - (\sigma_S - \sigma_C)}{\Delta_2}$\\
\\
For these bounds on $P_1$ to be consistent lower bound must be less than or equal to the upper bound on $P_1$.\\
$\frac{\sigma_S - \sigma_C}{\Delta_1} \geq \frac{\Delta_2 - (\sigma_S - \sigma_C)}{\Delta_2}$ $\implies \frac{\Delta_1 \Delta_2}{\Delta_1 + \Delta_2} \geq \sigma_S - \sigma_C$\\

We know that, $\frac{\Delta_1 \Delta_2}{\Delta_1 + \Delta_2} \geq \sigma_S - \sigma_I$ from \ref{equation_1} and $\sigma_S - \sigma_I \geq \sigma_S - \sigma_C$, thus $\frac{\sigma_S - \sigma_C}{\Delta_1} \geq \frac{\Delta_2 - (\sigma_S - \sigma_C)}{\Delta_2}$ $\implies \frac{\Delta_1 \Delta_2}{\Delta_1 + \Delta_2} \geq \sigma_S - \sigma_C$ always holds.\\
\\
Similarly, we find bounds on $P_2$,  $\frac{\sigma_S - \sigma_C}{\Delta_2} \leq P_2 \leq \frac{\Delta_1 - (\sigma_S - \sigma_C)}{\Delta_1}$\\
\\
\\ 
To find the optimal probability vector, we select the $P_k$ corresponding to the maximum coefficient equal to the lower bound on $P_k$ and pick $P_{-k} = 1 - P_K $. For example, if $\Delta_1 < \Delta_2$, $P_1 = \frac{\sigma_S - \sigma_C}{\Delta_2}$, and $P_2 = 1 - P_1$. 
It is crucial to see that $P_2 = 1 - P_1$, lies in the feasible range of $P_2$. as $1 - \frac{\sigma_S - \sigma_C}{\Delta_1} = \frac{\Delta_1 - (\sigma_S - \sigma_C)}{\Delta_1}$, which is same as the upper bound on $P_2$\\

\\
\\
CASE 2: If $\frac{\Delta_1 \Delta2}{\Delta_1 + \Delta2} < \sigma_s - \sigma_I$, then $P_I \neq 0$, i.e., payoff set corresponding to the strategy (I,I) is above the line joining payoffs for (T,I) and (I,T). It is clear from fig 1 that in this case the optimal lies on the line joining (I,T) and (I,I) or (T,I) and (I,I). So either $P_1$ or $P_2$ would be 0, depending upon the corresponding coefficients.

if $\Delta_1 > \Delta_2$, coefficient corresponding to $P_2 > P_1$, therefore we would minimize $P_2 = 0$ and $P_1 = 1 - P_I$. To find the probabilities with which each strategy is played, we simplify the constraints to:\\
\\
Constraint 1a:
$P_1(-\sigma_S) + P_2(-\Delta_1-\sigma_S) + P_I(-\Delta_1 - \sigma_I) \geq -\Delta_1 -\sigma_C$\\
$(1 - P_I)(-\sigma_S) + P_I(-\Delta_1 - \sigma_I) \geq -\Delta_1 -\sigma_C$\\
$\sigma_S + P_I(\Delta_1 - \sigma_S + \sigma_I) \leq \Delta_1 + \sigma_C$\\
$ P_I \leq \frac{\Delta_1 - \sigma_S + \sigma_C}{\Delta_1 - \sigma_S + \sigma_I}$\\
\\ 
Constraint 1b:
$P_1(-\Delta_2 -\sigma_S) + P_2(-\sigma_S) + P_I(-\Delta_2 - \sigma_I) \geq -\Delta_2 -\sigma_C$\\
$(1 - P_I)(\Delta_2 +\sigma_S) + P_I(\Delta_2 + \sigma_I) \leq \Delta_2 +\sigma_C$\\
$P_I \geq \frac{\sigma_S -\sigma_C}{\sigma_S -\sigma_I}$\\
\\
upper bound on $P_I$ should be greater than or equal to the lower bound on $P_I$. \\
$\frac{\Delta_1 - \sigma_S + \sigma_C}{\Delta_1 - \sigma_S + \sigma_I} > \frac{\sigma_S -\sigma_C}{\sigma_S -\sigma_I}$ \implies $\Delta_1\sigma_I < \Delta_1\sigma_C$ as $\sigma_C > \sigma_I$ this always holds.\\
To minimize the objective function, we minimize $P_I$ as coefficient corresponding to $P_I > P_1$, therefore we select $P_I = \frac{\sigma_S -\sigma_C}{\sigma_S -\sigma_I}$\\
Similarly if $\Delta_1 < \Delta_2$, $P_1 = 0$, $P_I = \frac{\sigma_S -\sigma_C}{\sigma_S -\sigma_I}$ and $P_2 = 1 - P_I$
\\
\\
\\
\textbf{N Player Game}: Similar to a 2-player game, we look for two different cases, one where the payoff point corresponding to strategy (I,I,..I) , i.e., all nodes sit idle lies above or below the plane including all the payoffs where one of the nodes successfully transmits. The equation of such a hyperplane is given by H(n,b) where $\Vec{n} = (\Delta_2\Delta_3...\Delta_N,  \Delta_1\Delta_3...\Delta_N, \Delta_1\Delta_2...\Delta_{N-1})$ is normal to the hyperplane and $b = \Vec{n} \times \Vec{x}$, and $\Vec{x}$ is some point on the hyperplane.\\ For example, a 3-player game has three payoff points $((-\sigma_S, -\Delta_2 - \sigma_S, -\Delta_3 - \sigma_S);(-\Delta_1 - \sigma_S, -\sigma_S, -\Delta_3 - \sigma_S); (\Delta_1 - \sigma_S, -\Delta_2 - \sigma_S, -\sigma_S))$ lying on the hyperplane. Let $\Vec{V_1V_2}$ and $\Vec{V_1V_3}$ be the vector from points 1(T,I,I) to 2(I,T,I) and 1(T,I,I) to 3(I,I,T), respectively.\\
\implies  $\vec{V_1V_2} = (\Delta_1, -\Delta_2, 0)$ and $ \Vec{V_1V_3} = (\Delta_1, 0, -\Delta_3)$, The normal vector is then given by the cross product of $\Vec{V_1V_2} \times \Vec{V_1V_3} = (\Delta_2\Delta_3, \Delta_1\Delta_3, \Delta1\Delta_2)$. Similarly, for N players, we find a normal vector to the N-1 hyperplane by the cross product of $(\Delta_1,-\Delta_2,0,0...,0); (\Delta_1,0,-\Delta_3,0,0,..,0);....;(\Delta_1,0,0,...,-\Delta_N)$

\\
\\
Case 1: $P_I = 0$, the optimization problem can be written as:
$Min_{P_K}$ $\sum_{k=1}^{N}(\Delta - \Delta_k +N\sigma_S)P_k$, where $\Delta = \sum_{k=1}^{N}\Delta_k$. Constrain 2 of the optimization problem states $\sum_{k=1}^{N}P_k = 1$.\\

Constraint 1: $\sigma_S P_k + (\Delta_k + \sigma_S)\sum_{j=1,j\neqk}^{N}P_j \leq \Delta_k + \sigma_C$, $\forall k \in N$ \implies $\sigma_S P_k + (\Delta_k + \sigma_S)(1 - P_k) \leq \Delta_k + \sigma_C$\\
\implies $P_k \geq \frac{\sigma_S - \sigma_C}{\Delta_k} $, $\forall k \in N$\\
\\
To allocate optimal probabilities, we select the node with the maximum age to transmit with the highest probability. For example, let $\Delta_1$ be the maximum age of a node in the network. Then, set the probabilities as $P_k = \frac{\sigma_S - \sigma_C}{\Delta_k}$ , and $P_1 = 1 - \sum_{k=2}^{N}P_k$


